Metric Learning for Image Registration

Image registration is a key technique in medical image analysis to estimate deformations between image pairs. A good deformation model is important for high-quality estimates. However, most existing approaches use ad-hoc deformation models chosen for mathematical convenience rather than to capture observed data variation. Recent deep learning approaches learn deformation models directly from data. However, they provide limited control over the spatial regularity of transformations. Instead of learning the entire registration approach, we learn a spatially-adaptive regularizer within a registration model. This allows controlling the desired level of regularity and preserving structural properties of a registration model. For example, diffeomorphic transformations can be attained. Our approach is a radical departure from existing deep learning approaches to image registration by embedding a deep learning model in an optimization-based registration algorithm to parameterize and data-adapt the registration model itself.

==> supplementary_material.tex <==
\section{Generating the synthetic test cases}

\begin{figure}
%\includegraphics[width=\textwidth]{figs/example_synthetic_case_generation/syncomb.pdf}
%\includegraphics[height=0.12\textheight]{figs/example_synthetic_case_generation/cropped-std_im_source_0.pdf}
%\includegraphics[height=0.12\textheight]{figs/example_synthetic_case_generation/cropped-random_source_m_smoothed_orig_0.pdf}
%\includegraphics[height=0.12\textheight]{figs/example_synthetic_case_generation/cropped-source_image_0.pdf}
%\includegraphics[height=0.12\textheight]{figs/example_synthetic_case_generation/cropped-std_im_orig_0.pdf}
%
  \begin{tabular}{llll}
    %\includegraphics[width=0.475\textwidth]{figs/example_synthetic_case_generation/cropped-ring_im_orig_0.pdf} &
    (a) & 
    \includegraphics[height=0.225\textheight]{figs/example_synthetic_case_generation/cropped-circle_init_m_smoothed_orig_0.pdf} &
    %\includegraphics[width=0.475\textwidth]{figs/example_synthetic_case_generation/cropped-ring_im_warped_source_0.pdf} \\
    (b) & \includegraphics[height=0.225\textheight]{figs/example_synthetic_case_generation/cropped-random_source_m_smoothed_orig_0.pdf} \\
    (c) & \includegraphics[height=0.225\textheight]{figs/example_synthetic_case_generation/cropped-source_image_0.pdf} &
    (d) & \includegraphics[height=0.225\textheight]{figs/example_synthetic_case_generation/cropped-target_image_with_grid_0.pdf} \\
    (e) & \includegraphics[height=0.225\textheight]{figs/example_synthetic_case_generation/cropped-std_im_orig_0.pdf} &
    (f) & \includegraphics[height=0.225\textheight]{figs/example_synthetic_case_generation/cropped-std_im_source_0.pdf}
  \end{tabular}
  \caption{Illustration of the intermediate steps during synthetic test case generation, as described in Sect.~\ref{subsec:synthetic_experiment_setup}. %This example shows the generation of one \emph{source} image.} 
  (a) A shape with concentric circles and a smoothed momentum field (based on a random unsmoothed momentum field on the edges of the shape) is generated (randomly); (b) the momentum from (a) results in a deformed shape. This shape is considered the \emph{source} image. Again, a random smoothed momentum field is generated; (c) Random noise is added to the source image and it is deformed based on the momentum in (b) to result in the textured target image (d). Each ring has a different multi-Gaussian weight. The resulting standard deviations of the original concentric shape of (a) and of the generated source image in (c) are shown in (e) and (f), respectively.}
  \label{fig:example_generation}
\end{figure}


